Reinforcement Learning for Automatic Test Case Prioritization and Selection in Continuous Integration

Testing in Continuous Integration (CI) involves test case prioritization, selection, and execution at each cycle. Selecting the most promising test cases to detect bugs is hard if there are uncertainties on the impact of committed code changes or, if traceability links between code and tests are not available. This paper introduces Retecs, a new method for automatically learning test case selection and prioritization in CI with the goal to minimize the round-trip time between code commits and developer feedback on failed test cases. The Retecs method uses reinforcement learning to select and prioritize test cases according to their duration, previous last execution and failure history. In a constantly changing environment, where new test cases are created and obsolete test cases are deleted, the Retecs method learns to prioritize error-prone test cases higher under guidance of a reward function and by observing previous CI cycles. By applying Retecs on data extracted from three industrial case studies, we show for the first time that reinforcement learning enables fruitful automatic adaptive test case selection and prioritization in CI and regression testing.

==> preamble.tex <==
\newcommand{\includeBigFigures}      {true}
\newcommand{\insertEmptyFig}      {\missingfigure[figwidth=\textwidth]{Missig figure, Set includeBigFigures to true to include figure}}

\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\expref}[1]{Exp#1}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{#1}}
\newcommand{\listref}[1]{Listing~\ref{#1}}







% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}


\definecolor{gray1}{gray}{0.8}
\definecolor{gray2}{gray}{0.85}
\definecolor{gray3}{gray}{0.75}
\definecolor{gray4}{gray}{0.65}

%#1=taskname, #2=machineNo, #3=Start, #4= duration, #5=color
\newcommand{\drawschedule}[5]	
{
	begin{scope}
	{
		\draw[fill=#5] (#3,#2-\mshift) rectangle (#4+#3,#2+\task_h-\mshift);
		\node at (#3+#4*0.5,#2+0.5*\task_h-\mshift) {$#1$};
	}
}

%#1=file
%#2=maxnum
%\newcommand{\solvegraph}[2]	
%{
%	\begin{tikzpicture}
%	
%		\begin{axis}[
%				title={#1},
%				width=\linewidth,
%				xlabel={Solving time},
%				%xlabel near ticks,
%				ylabel={Max span},
%				%ylabel near ticks,
%				%legend columns=1,
%				%legend style={at={(0.8,-0.3)},font=\tiny}]
%				%,
%				%anchor=north,legend columns=3},
%				mark size=1.0]
%	
%			\foreach \i in {1,...,#2}
%			{
%				%\addplot table[x=stime, y=etimemax] {#1_\i.dat};
%				\addplot table[] {#1_\i.dat};
%			}
%%
%%		%\legend
%%		%{?
%%		%	{$H_1$,\btabsize=10},
%%		%	{$H_2$,\btabsize=10},
%%		%	{$H_1$,\btabsize=40},
%%		%	{$H_2$,\btabsize=40}
%%		%}
%%	
%		\end{axis}
%	\end{tikzpicture}
%}
%                                            

\newcommand{\plotmaxspan}[1]{
% \begin{figure}
% \centering
	\begin{tikzpicture}
		\begin{axis}[
				title={#1},
				width=\linewidth,
				xlabel={Solving time},
				ylabel={Max span},
				%ytick={0,10000,20000,30000},
				%yticklabels={0,10,20,30},
				%xtick={1,10,30,60,300,900},
				%xticklabels={1,10,30,60,300,900},
				mark size=0.0]
				\addplot table[] {data/defaultlabeling/#1};
				\addplot table[] {data/circularlabeling/#1};
				\legend{Default,Circular}
		\end{axis}
	\end{tikzpicture}
	\\
% \caption{Caption}
% \end{figure}
}

%Hein@Morten ^: I commented the figure float, because it was causing problems too. The macro may work when plotting fewer plots. Not sure exactly why it doesn't work with many plots. There are some latex parameters that can be tuned but I don't remember which params it would be and if it would work. (Consider this solution a workaround for now. I expect we won't be plotting so many plots in the final version of the paper, and hopefully it will be able to compile with the necessary plots without problems.)



%Settings for boxplot:
\pgfplotsset{
    box plot/.style={
        /pgfplots/.cd,
        black,
        only marks,
        mark=-,
        mark size=1em,
        /pgfplots/error bars/.cd,
        y dir=plus,
        y explicit,
    },
    box plot box/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \draw  ##1 -- ++(1em,0pt) |- ##2 -- ++(-1em,0pt) |- ##1 -- cycle;
        },
        /pgfplots/table/.cd,
        y index=2,
        y error expr={\thisrowno{3}-\thisrowno{2}},
        /pgfplots/box plot
    },
    box plot top whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=4,
        y error expr={\thisrowno{2}-\thisrowno{4}},
        /pgfplots/box plot
    },
    box plot bottom whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=5,
        y error expr={\thisrowno{3}-\thisrowno{5}},
        /pgfplots/box plot
    },
    box plot median/.style={
        /pgfplots/box plot
    }
}

